PIE: Simulating Disease Progression via Progressive Image Editing

Disease progression simulation is a crucial area of research that has significant implications for clinical diagnosis, prognosis, and treatment. One major challenge in this field is the lack of continuous medical imaging monitoring of individual patients over time. To address this issue, we develop a novel framework termed Progressive Image Editing (PIE) that enables controlled manipulation of disease-related image features, facilitating precise and realistic disease progression simulation. Specifically, we leverage recent advancements in text-to-image generative models to simulate disease progression accurately and personalize it for each patient. We theoretically analyze the iterative refining process in our framework as a gradient descent with an exponentially decayed learning rate. To validate our framework, we conduct experiments in three medical imaging domains. Our results demonstrate the superiority of PIE over existing methods such as Stable Diffusion Walk and Style-Based Manifold Extrapolation based on CLIP score (Realism) and Disease Classification Confidence (Alignment). Our user study collected feedback from 35 veteran physicians to assess the generated progressions. Remarkably, 76.2% of the feedback agrees with the fidelity of the generated progressions. To our best knowledge, PIE is the first of its kind to generate disease progression images meeting real-world standards. It is a promising tool for medical research and clinical practice, potentially allowing healthcare providers to model disease trajectories over time, predict future treatment responses, and improve patient outcomes.

==> tex_files/background.tex <==
% \section{Background}
% \textbf{Denoising Diffusion Probabilistic Models} (DDPM) ~\citep{ho2020denoising} are a class of generative models that use a diffusion process to transform a simple initial distribution, such as a Gaussian, into the target data distribution. The model assumes that the data points are generated by iteratively applying a diffusion process to a set of latent variables $x_1, \ldots, x_T$ in a sample space $\chi$. At each time step $t$, Gaussian noise is added to the latent variables $x_t$, and the variables are then transformed back to the original space using a learned invertible transformation function. This process is repeated for a fixed number of steps to generate a final output. The latent variable models can be expressed in the following form,  
% \begin{equation}
%     p_\theta(x_0) = \int p_{\theta}(x_{0:T})dx_{1:T}, \ \ \ \ where\ \ \ p_{\theta}(x_{0:T})\prod_{t = 1}^{T}p_{\theta}^{(t)}(x_{t - 1} | x_t)
%     \label{eq:background:1}
% \end{equation}
% Because of a special property of the forward process,
% \begin{equation}
%     q(x_t|x_0) = \int q(x_{1:t} | x_0) dx_{1:(t-1)} = \mathcal{N}(x_t; \sqrt{\alpha_t} x_0, (1 - \alpha_t)\cdot \mathbf{I})
%     \label{eq:background:2}
% \end{equation}
% we can express $x_t$ as a linear combination of $x_0$ and a noise variable $\epsilon$, which is the key to enabling the image editing process.
% \begin{equation}
%     x_t = \sqrt{\alpha_{t}}\cdot x_{0} + \sqrt{1 - \alpha_{t}} \cdot \epsilon, \ \ \ \ where \ \ \ \ \epsilon \sim \mathcal{N}(\mathbf{0}, \mathbf{I})
%     \label{eq:background:3}
% \end{equation}

% \textbf{Denoising Diffusion Implicit Models} (DDIM) ~\citep{song2020denoising} that uses a non-Markovian forward process to generate data. Unlike Denoising Diffusion Probabilistic Models (DDPM), DDIM does not require explicit modeling of the latent variables. Instead, the model generates samples by solving a non-linear differential equation, which defines a continuous-time evolution of the data distribution. We can express its forward process as follows,
% \begin{equation}
%     q_{\sigma} (x_{1:T} | x_0):= q_{\sigma}(x_T | x_0) \prod_{t = 2}^T q_{\sigma}(x_{t - 1}| x_t, x_0)
%     \label{eq:background:4}
% \end{equation}
% where $q_{\sigma} (x_{t-1}| x_t, x_0) = \mathcal{N}(\sqrt{\alpha_T}x_0, (1 - \alpha_T), \mathbf{I})$ and for all $t > 1$
% \begin{equation}
%     q_{\sigma}(x_{t - 1} | x_t, x_0) = \mathcal{N} (\sqrt{\alpha_{t - 1} x_0} + \sqrt{1 - \alpha_{t - 1} - \sigma_t^2}\cdot \frac{x_t - \sqrt{\alpha_t}x_0}{\sqrt{1 - \alpha_t}}, \sigma_t^2 \mathbf{I})
%     \label{eq:background:5}
% \end{equation}
% Setting $\sigma_t = 0$, it defines a generation process going from $x_{t}$ to $x_{t - 1}$ as follows
% \begin{equation}
%     x_{t - 1} = \sqrt{\alpha_{t - 1}} (\frac{x_t - \sqrt{1 - \alpha_t} \epsilon_{\theta}^{(t)}(x_t)}{\sqrt{\alpha_t}}) + \sqrt{1 - \alpha_{t - 1}}\cdot \epsilon^{(t)}_{\theta}(x_t)
%     \label{eq:background:6}
% \end{equation}
% where the $\epsilon_{\theta}^{(t)}(x_t)$ is a model that attempts to predict $\epsilon_t \sim \mathcal{N}(\mathbf{0}, \mathbf{I})$ from $x_t$

% \textbf{Guided Image Editing via Diffusion} ~\citep{meng2021sdedit,lugmayr2022repaint,couairon2022diffedit} are general techniques that aim to modify either the entirety or certain parts of images through diffusion. The process commences by introducing noise to the genuine base image and subsequently applying the reverse diffusion process to remove the noise, resulting in the production of photo-realistic images. Specifically, we employ the DDIM forward process \ref{eq:background:3} for the addition of noise and the reverse process \ref{eq:background:6} for one cycle of image modification, as demonstrated in \ref{algo:1}.

